Non-euclidean shadows of classical projective theorems

Some translations into non-euclidean geometry of classical theorems of planar projective geometry are explored. The existence of some common triangle centers is dedeuced from theorems of Pascal and Chasles. Desargues' Theorem allows to construct a non-euclidean version of the Euler line and the nine-point circle of a triangle. The whole non-euclidean trigonometry (for triangles and generalizaed triangles) can be deduced from Menelaus' Theorem. A theorem of Carnot about affine triangles implies the non-euclidean versions of another theorem of Carnot about euclidean triangles. Finally, it is given the projective theorem which is hidden behind all the laws of cosines of non-euclidean triangles and generalized triangles.

==> theBibligraphy.tex <==
\bibitem{Akopyan-other-proposal}Arseniy V. Akopyan, \emph{On some
classical constructions extended to hyperbolic geometry}, http://arxiv.org/abs/1105.2153

\bibitem{Baker} Baker, H. F., \textit{Principles of Geometry}, 2nd Ed., Cambridge Universty Press 1930.

\bibitem{Beardon} Beardon, A. F., \textit{The Geometry of Discrete
Groups}, New york, 1983.

% \bibitem{Bonola} Bonola, R.,\textit{ La geometria non-euclidea},
% Bologna, 1906.

\bibitem{Buser} Buser, P., \textit{Geometry and Spectra of Compact
Riemann Surfaces}, Boston, 1992.

\bibitem{Cayley} Cayley, A., \textit{A sixth memoir upon quantics},
Philosophical Transactions of the Royal Society of London, 149 (1859),
pp. 61-90.

\bibitem{Coolidge} Coolidge, J. L., \textit{The elements of non-euclidean geometry}, Oxford, At the Clarendon press, 1909.

\bibitem{Cox Proj} Coxeter, H. S. M., \textit{The Real Projective
Plane}, Cambridge, 1955.

\bibitem{Cox Non-euc} Coxeter, H. S. M.,\textit{ Non-euclidean geometry},
Toronto, 1968.

\bibitem{Demirel-Soyturk}Demirel, O. and Soyt{\"u}rk, E., \textit{The hyperbolic Carnot theorem in the Poincar\'e disc model of hyperbolic geometry}, Novi Sad J. Math.  38 (2008), no. 2, 33–39.

% \bibitem{Enriques} Enriques, F., \textit{Lezioni di Geometria Proiettiva},
% Bologna, 1904.

\bibitem{Fenchel}Fenchel, W., \emph{Elementary Geometry in Hyperbolic
Space}, Berlin, 1989.

\bibitem{Forder} Forder, H. G., \textit{The cross and the foundations
of euclidean geometry}, Mathematical Gazette, 31 (1947), pp. 227-233.

\bibitem{GeoGebra}
Hohenwarter, M.,
\textit{GeoGebra: Ein Softwaresystem f\"ur dynamische Geometrie und
Algebra der Ebene},
Master Thesis, Paris Lodron University, Salzburg, Austria, 2002. Software
currently developed by IGI, http://www.geogebra.org.

\bibitem{Johnson} Johnson, \textit{Directed angles in elementary
geometry}, American Mathematical Monthly, 24 (1917), pp. 101-105.

\bibitem{Klein} Klein, F., \textit{Ueber die sogenannte Nicht-Euklidische
Geometrie}, Mathematische Annalen, 4 (1871), pp. 573-625. English
translation in \cite{Stillwell}.

\bibitem{Laguerre} Laguerre, E., \textit{Note sur la théorie des
foyers}, Nouvelles Annales de Mathématiques, 12 (1853), pp. 57-66.

% \bibitem{Milnor} Milnor, J., \textit{Hyperbolic geometry: The first
% 150 years}, Bulletin of the American Mathematical Society, 6 (1982),
% pp. 9-24.

\bibitem{Picken} Picken, D. K.,\textit{ Euclidean geometry of angle},
Proceedings of the London Mathematical Society, (2) vol. 23 (1925),
pp. 45-55.

\bibitem{Plato} Plato, \textit{The Republic: Allegory of the Cave.}

\bibitem{Richter-Gebert}Richter-Gebert, J., \emph{Perspectives on
projective geometry. A guided tour through real and complex geometry},
Springer, Heidelberg, 2011.

\bibitem{Santalo} Santal\'o, L., \textit{Geometr\'{i}as no euclidianas},
Buenos Aires, 1961.

% \bibitem{Sarli} Sarli, J., \textit{Conics in the hyperbolic plane intrinsic to the collineation group}, Journal of Geometry  103 (2012), no. 1, 131–148.

\bibitem{Stillwell} Stillwell, J., \textit{Sources of Hyperbolic
Geometry}, AMS., 1996.

\bibitem{Thurston} Thurston, W.P., \textit{Three-dimensional geometry
and topology}, Princeton, 1997.


\bibitem{V - Y} Veblen and Young, \textit{Projective Geometry}: vol.
I, Boston, 1910; vol. II, 1918.

\bibitem{Wildberger} Wildberger, N. J., \emph{Universal hyperbolic
geometry II: a pictorial overview}, KoG 14 (2010), 3-24.

\bibitem{Wildberger2} Wildberger, N. J., \emph{Universal hyperbolic
geometry III: first steps in projective triangle geometry}, KoG 15 (2011), 25-49.

